A Novel Approach for Attack Tree to Attack Graph Transformation: Extended Version

Attack trees and attack graphs are both common graphical threat models used by organizations to better understand possible cybersecurity threats. These models have been primarily seen as separate entities, to be used and researched in entirely different contexts, but recently there has emerged a new interest in combining the strengths of these models and in transforming models from one notation into the other. The existing works in this area focus on transforming attack graphs into attack trees. In this paper, we propose an approach to transform attack trees into attack graphs based on the fundamental understanding of how actions are represented in both structures. From this, we hope to enable more versatility in both structures.

==> content/Evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}
% Use the run in example / SAND attack tree - what can we learn from it
% This is the "So What" section
% Look for papers where they have a transformation schema/technique for attack graphs
% Hand wavy is okay
% Intoduce notion of system
% Working with Human designed attack trees would already be interesting



If we return to the example found in Section \ref{sec:example}, we can see that the application of the algorithm as described on Figure~\ref{fig:AttackTree} will exactly result in the attack graph shown in Figure~\ref{fig:AttackGraph}. For every attack vector represented in the attack tree, the same attack vector is represented similarly in the attack graph, only with the introduction of states. These states are not provided with specific meaning outside of numbering as our specific definition; however, the ability to assign further meaning to these states is not excluded by our methodology. 

\paragraph{Enabling broader generation schemes.}

Most attack trees are human generated, and if attack graphs would similarly need to be human generated, as discussed by Valmari, the number of states would be unwieldy \cite{valmariStateExplosionProblem1998}. As such, it is impractical for a human to generate an attack graph that would be large enough to be of practical use; however, by enabling the transformation from a human generated attack tree to a transformed attack graph, we create an attack graph structure that is still usable by humans without the necessity for a human to manually produce a subsequent attack graph.

Another advantage of enabling a direct transformation between attack trees and attack graphs is that new, automated generation schemes for attack graphs become possible. As we discussed above, significant research has already been performed into novel generation schemes for attack trees. A major branch of current attack tree research is into generation schema, particularly focusing on automated machine generation. Therefore, one advantage of being able to transform attack trees into attack graphs is the ability to use these novel generation methods to generate attack graphs.



\paragraph{Bijective mapping.}

While the transformation discussed here is in a single direction, as we discussed in Section~\ref{sec:defs}, we deliberately use the same definition of attack graphs as Pinchinat \et\ in their work on the ATSyRa algorithm which transforms attack graphs into attack trees \cite{pinchinatATSyRaIntegratedEnvironment2016}. As such, the attack graphs generated from our algorithm could be used as input into the ATSyRa algorithm to return them to attack trees.

This potentially enables the ability to convert an attack tree into an attack graph, the manipulation of the attack graph, and then conversion back into an attack tree. Furthermore, we now have a greater means to study potential edge cases within these models, for instance, the introduction of cycles within an attack graph, or the removal of a given state or specific attack vector.

\paragraph{Expansion of the transformation schema.}

Thus far we have only concerned ourselves with a simple SAND attack tree \cite{jhawarAttackTreesSequential2015}, but further expansion of attack trees are avaliable. For instance, we could expand this transformation to use an attack defense tree (AD Tree) as an input, and then created an expanded attack graph representing the defensive actions represented in the attack tree. Expansion of the transformation methodology in this vein would similarly apply to the attack graph to attack tree ATSyRa transformation \cite{pinchinatSynthesisAttackTrees2014}.


==> content/TransformationOLD.tex <==
\section{Transformation}
\label{sec:transformation}

Examining any attack tree, we can see that the nodes represent individual attack components, or in the case of the overall root, the overarching goal of the attack. The edges of an attack tree represent a connection relationship between individual attack components; in a basic attack tree, this is the only information contained within the edges. By contrast, edges in attack graphs arguably contain attack components [CITATION NEEDED]. The edges represent transition relations between attack states, stored in nodes. This brings us to our first insight, nodes in attack trees will have to be mapped to edges in attack graphs.

If we consider the entire structure of the attack tree, we see that the overall goal is at the top in the root node, and the leaves farthest from the root represent the first components of any attack vector [CITATION NEEDED - Maybe Mauw or Schneier]. The common understanding of attack trees is that they "flow" from bottom to top [CITATION NEEDED]. In the attack graph, this overall structure is reversed. The starting states are generally organized at the top, While the success states are organized at the bottom. In a state based attack graph, the "flow" is from the starting states to the success states, or from top to bottom. This brings us to the second insight, we need to "flip the flow" when converting between attack graphs and attack trees.

When we combine these two insights, we begin to find a macro-strategy to transform an attack tree into an attack graph. We will need a direct mapping of nodes to edges, in a methodology that is continually repeatable so as not to create an infinite series of edge cases such that a common transformation scheme would be undefinable. Additionally, we will have to ensure that this application of continually repeatable steps does not result in a tangled web of edge cases. Finally, we will have to take measures to limit the number of potential states in the attack graph given that the state expansion problem will result in an unmanageably large graph.


By combining the insights we have found thus far, we can begin to define an algorithm to convert from attack trees to attack graphs.

\begin{enumerate}
\item Compress the attack tree along base elements
\item Build the attack graph as we expand the attack tree
\item Repeat until no compressed elements remain
\end{enumerate}

As was mentioned, there is need for a mechanism to reverse the "flow" of the attack model when transforming between attack graphs and attack trees. This mechanism is compression and expansion. With compression, we slowly reduce attack tree until it is a single node. A single node cannot carry directional information, and as such can be thought of as either having no "flow" or bidirectional "flow". Once we have accomplished removing "flow" in one direction, we can then expand the tree, and as we expand, we can systematically build a graph "flowing" in the opposite direction. While the same goal may be achievable with a mechanism other than compression and expansion, the mechanism provided below works as a formal method to describe this "flow" reversal for both directions of the transformation.


%\subsection{Initialization}

%We start with a single starting node on the attack graph. While attack graphs specifically allow for multiple origin nodes, we deliberately exclude this possibility for simplicity. This exclusion is specifically addressed in the Considerations Section below. We initialize the attack graph with a single node, as this node needs to exist in order to build off of this node. Additionally, we mark this node in the attack graph with the $T_0$ origin marker. These origin markers will be used later to determine where edges and nodes should be placed. Finally, we initialize the attack tree, by adding the origin marker $T_0$ to all leaf nodes.


%\subsection{Adding AT elements to AG}
\subsection{Compressing the attack tree}

As was defined in section \ref{sec:defs}, we recognize three radical elements of attack trees. The specific definitions of these radicals are found in definitions \ref{def:AND}, \ref{def:OR}, and \ref{def:SINGLE}.  These radicals will be individually compressed to single nodes. This compression does not remove any information from the attack tree. Rather, the compression is a formality to enable to compression of the tree as a whole. The compression can also be thought of as a grouping step, where the radical is grouped as a subtree, and the  connection from the overall attack tree is redefined from a connection with the radical itself to a connection with the radical subtree.


We start the algorithm by examining leaf radicals. A leaf radical is a radical such that only the root of the radical is a parent node, all other nodes in the radical are leaf nodes, that is to say, all other nodes in the radical have no children. Every compression step of this algorithm starts with a leaf radical. The leaf radical is compressed to a single node, labeled $T_i$ where $i$ is the number of compressions performed. This node, $T_i$, is a subtree containing a single radical, and takes the place previously held by the root of the radical stored in $T_i$. The remaining tree will either have another leaf radical, or be reduced to a single node. If the tree is more than a single node, this compression step repeats, with previous compressions treated as nodes. Once the attack tree is completely compressed to a single node, we move onto the expansion step.








\subsection{Expanding the tree and building the attack graph}

After we have compressed the attack tree to a single node, we then expand the attack tree and build the attack graph along the expansion. We have a defined mapping from attack tree radicals to attack graph radicals. The compression has enabled us to consider a single radical per expansion step, allowing us to build an attack graph with only three defined mappings. If we were to try to expand this mapping, we would quickly find the state expansion problem would create an unwieldy number of mappings and edge cases [CITATION NEEDED], thus that the algorithm is less a systematic process to transform attack trees to attack graphs, and more a large dictionary of premapped complete attack trees and attack graphs.

We initialize the attack graph with a single starting state $S_0$ and a single success state $S_s$. While the attack graph definition that we are using from Sheyner allows for a set of starting and success states, we assume that these sets contain a single item [CITE SHEYNER]. This assumption is addressed in the considerations section. Additionally, our attack graph has a single transition defined as $T_j$ where $j$ is the total number of distinct compressions from the attack tree compression step.

After we have initialized the attack graph, we then begin expanding. \marginpar{Do I need to prove this? If I do, what kind of proof does this form take?} Attack graph transitions labeled as $T_i$ are subtransitions, which need to be expanded. These expansions depend on the radical being represented by $T_i$.
Below, we have our defined radical maps. The same information represented in attack trees is additionally represented in attack trees.


\subsubsection{OR Radical}

Our understanding of the \OR radical in attack trees is that only a single component of an \OR radical needs to be completed in order for the goal, or root, of the \OR to also be accomplished. This is expressed as separate components individually attached to the overall goal. As such, in an attack graph where individual attack vectors are expressed more explicitly, we would expect that each individual component would contribute to a separate attack vector. These separate attack vectors would result in separate states in the attack graph, as each attack component is a different state transition, and different state transitions result in different states.


\begin{figure}[h!]
  \centering
  \begin{forest}
    for tree={
      draw,
      minimum height=1cm,
      anchor=parent,
      align=center,
      child anchor=parent,
      edge=<-
    },
    adnode/.style={rounded rectangle,},
      [{Goal}, adnode, %angle below
        [{Attack\\Component 1}, adnode]
        [{$\hdots$}, adnode]
        [{Attack\\Component $n$}, adnode]
      ]
  \end{forest}
\label{fig:OR_AT_rad}
\caption{OR Radical in an Attack Tree}
\end{figure}


\begin{figure}[h!]
  \centering
  \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto, node distance=3.2cm,
                      semithick]
    \tikzstyle{every state}=[fill=white,draw=black,text=black]

    \node[state, draw=none] (0) [below left of=0] {};
    \node[state]         (1) [below left of=0] {$S_1$};
    \node[state]         (n) [below right of=0] {$S_n$};
    \node[state]         (2) at ($(1)!0.5!(n)$) {$S_k$};
    \node[state, draw = none]         (5) [below of=1]  {};
    \node[state, draw = none]         (8) [below of=n]  {};
    \node[state, draw = none]         (7) at ($(5)!0.5!(8)$)  {};


    \path (0) edge              node [left]{Attack Component 1} (1)
              edge              node {$\hdots$} (2)
              edge              node [right]{Attack Component $n$} (n)
          (n) edge node {Goal} (8)
          (2) edge node {Goal} (7)
          (1) edge node {Goal} (5);

  \end{tikzpicture}
\label{fig:OR_AG_rad}
\caption{OR Radical in an Attack Tree}
\end{figure}


As we can see in Figure \ref{fig:OR_AG_rad}, the \OR radical in an attack graph is a series of disjoint ``legs'' with a state transition culminating in a state for each attack component represented in the attack tree. As each attack component is unique, the system states that are a result of application of those attack components must also be unique. This does not rule out the possibility of the application of unique attack components resulting in the same state; that would be a possible expansion of the radical mapping we have laid out here. Given that the goal in a radical could itself be a component in another radical, we see that the goal in the attack tree radical is again represented as a state transition in the attack graph.



an OR radical creates a series of disjoint "legs" in the attack graph. Given that only one component in the OR radical needs to be completed for that radical to have a successful attack, we only need to consider states created by following each component individually. This means we will result in a total of $n$ states in the attack graph. We assume that only one component in the OR relationship will ever be followed in a single attack vector. This assumption is addressed in \ref{ssec:xor}




\subsubsection{AND Radical}
\label{ssec:AND}

\begin{figure}
  \centering
  \begin{forest}
    for tree={
      draw,
      minimum height=1cm,
      anchor=parent,
      align=center,
      child anchor=parent,
      edge=<-
    },
    adnode/.style={rounded rectangle,},
      [{Goal}, adnode, angle below
        [{Attack\\Component 1}, adnode]
        [{$\hdots$}, adnode]
        [{Attack\\Component $n$}, adnode]
      ]
  \end{forest}


  \label{fig:AND_AT_rad}
\caption{AND Radical}
\end{figure}
\begin{figure}[h!]
  \centering
  \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto, node distance=3cm,
                      semithick]
    \tikzstyle{every state}=[fill=white,draw=black,text=black]

    \node[state, draw=none] (0) [below left of=0] {};
    \node[state]         (1) [below left of=0] {$S_1$};
    \node[state]         (3) [below right of=0] {$S_n$};
    \node[state]         (2) at ($(1)!0.5!(3)$) {$S_k$};
    \node[state]         (4) [below left  of=1] {$S_{n+1}$};
    \node[state]         (6) [below right of=3] {$S_{n\choose{2}}$};
    \node[state]         (5) at ($(4)!0.5!(6)$) {$S_{n+k}$};
    \node         (Ml) [below=.5cm of 4 ] {};
    \node         (Mr) [below= .5cm of 6 ] {};
    \node         (M) [below= .5cm of 5 ] {\Huge$\hdots$};
    %\node[state]         (7) [below  of=Ml] {$S_{\sum_{j=1}^{n-2}{n\choose{j}}}$};
    \node[state]         (7) [below=.7cm of Ml] {$S_{2^n - (n+2)}$};
    \node[state]         (9) [below= .7cm of Mr] {$S_{2^n-2}$};
    \node[state]         (8) at ($(7)!0.5!(9)$) {$S_{2^n - (n+2) + k}$};
    \node[state]         (10) [below of=8] {$S_{2^n - 1}$};
    \node         (G) [below of=10 ] {};
    % \node[state, draw = none]         (6) [below of=3]  {};
    % \node[state, draw = none]         (8) [below of=4]  {};
    % \node[state, draw = none]         (7) at ($(6)!0.5!(8)$)  {};


    \path (0) edge              node [left]{Attack Component 1} (1)
              edge              node {$\hdots$} (2)
              edge              node [right]{Attack Component $n$} (3)
          (1) edge              node [left]{$\hdots$} (4)
              edge              node {$\hdots$} (5)
          (2) edge              node [sloped,] {Attack Component 1} (4)
              edge              node [sloped,] {Attack Component $n$} (6)
          (3) edge              node {$\hdots$} (5)
              edge              node [right]{$\hdots$} (6)
          (7) edge              node [sloped,]{Attack Component $n$} (10)
          (8) edge              node {$\hdots$} (10)
          (9) edge              node [sloped,]{Attack Component 1} (10)
          (10)edge              node {Goal} (G);
          % (n) edge node {Goal} (8)
          % (2) edge node {Goal} (7)
          % (1) edge node {Goal} (6);

  \end{tikzpicture}
\label{fig:AND_AG_rad}
\caption{\AND Radical in an Attack Graph}
\end{figure}









\begin{itemize}

% \item\textbf{Single Radical}
% As we can see in Figure \ref{fig:single_rad}, a single element radical in an attack tree forms a simple passthrough state in an attack graph. Given that the attack component in the attack tree is a single attack element attached to its parent element, in the attack graph, this is represented as a simple, single transition from one state to the next. The single element radical can be though of as a 1-element OR relationship, however for clarity, it is included as a separate classification here. \marginpar{Should I removed a defintion of single element radicals, and only have 2 radicals?}

\item\textbf{AND Radical}
As we can see in Figure \ref{fig:AND_rad}, an AND radical creates a lattice structure in the attack graph. With AND components, we must eventually use every defined component in attack trees. As such, in attack graphs, we will ultimately arrive at the same state. This assumes that the order of components does not matter, \textit{i.e.}, applying attack component $a$ then $b$ will have the exact same result as applying $b$ then $a$. This assumption is addressed is section \ref{ssec:sand}. The lattice structure is created in rows, starting with a single state for all components of the AND (a row of $n$ states given $n$ components in the and). The second row, will connect all possible combinations of 2 components, or $n\choose{2}$ possible states. This repeats until we are left with a single state that is the combination of all possible components of the and $n\choose{2} = 1$. The total number of states in the attack graph AND radical is $2^n$ where $n$ is the number of individual components in the AND radical.


\item\textbf{OR Radical}
As we can see in Figure \ref{fig:OR_rad}, an OR radical creates a series of disjoint "legs" in the attack graph. Given that only one component in the OR radical needs to be completed for that radical to have a successful attack, we only need to consider states created by following each component individually. This means we will result in a total of $n$ states in the attack graph. We assume that only one component in the OR relationship will ever be followed in a single attack vector. This assumption is addressed in \ref{ssec:xor}


\end{itemize}








\begin{comment}
\begin{figure}
\begin{subfigure}{0.5\textwidth}
  % \centering
  % \includegraphics[width=.4\linewidth, keepaspectratio]{img/AT_radical_AND.png}
  \resizebox{150pt}{75pt}{
  \begin{forest}
    for tree={
      draw,
      minimum height=1cm,
      anchor=parent,
      align=center,
      child anchor=parent,
      edge=<-
    },
    adnode/.style={rounded rectangle,},
      [{Goal}, adnode, angle below
        [{Attack\\Component 1}, adnode]
        [{$\hdots$}, adnode]
        [{Attack\\Component 2}, adnode]
      ]
  \end{forest}
  }

  \caption{Attack Tree}
  \label{sfig:AT_AND_rad}
\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \resizebox{150pt}{150pt}{
  % \centering
  % \includegraphics[width=.4\linewidth, keepaspectratio]{img/AG_radical_AND.png}
  \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto, node distance=3.2cm,
                      semithick]
    \tikzstyle{every state}=[fill=white,draw=black,text=black]

    \node[state, draw=none] (0) [below left of=0] {};
    \node[state]         (2) [below left of=0] {$S_1$};
    \node[state]         (1) [below right of=0] {$S_2$};
    \node[state]         (5) [below right of=2]  {$S_3$};
    \node[state, draw = none]         (8) [below of=5]  {};

    \path (0) edge              node [right]{Attack Component 1} (1)
              edge              node [left]{Attack Component 2} (2)
          (1) edge node {Attack Component 2} (5)
          (2) edge node [left]{Attack Component 1} (5)
          (5) edge node {Goal} (8);

  \end{tikzpicture}
  }
  \caption{Attack Graph}
  \label{sfig:AG_AND_rad}
\end{subfigure}
\caption{AND Radical}
\label{fig:AND_rad}
\end{figure}



\begin{figure}
\begin{subfigure}{.5\textwidth}
  % \centering
  % \includegraphics[width=.4\linewidth, keepaspectratio]{img/AT_radical_AND.png}
  \resizebox{150pt}{75pt}{
  \begin{forest}
    for tree={
      draw,
      minimum height=1cm,
      anchor=parent,
      align=center,
      child anchor=parent,
      edge=<-
    },
    adnode/.style={rounded rectangle,},
      [{Goal}, adnode, %angle below
        [{Attack\\Component 1}, adnode]
        [{Attack\\Component 2}, adnode]
      ]
  \end{forest}
  }
  \caption{Attack Tree}
  \label{sfig:AT_OR_rad}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  % \centering
  % \includegraphics[width=.4\linewidth, keepaspectratio]{img/AG_radical_AND.png}
  \resizebox{150pt}{130pt}{
  \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto, node distance=3.2cm,
                      semithick]
    \tikzstyle{every state}=[fill=white,draw=black,text=black]

    \node[state, draw=none] (0) [below left of=0] {};
    \node[state]         (2) [below left of=0] {$S_1$};
    \node[state]         (1) [below right of=0] {$S_2$};
    \node[state, draw = none]         (5) [below of=1]  {};
    \node[state, draw = none]         (8) [below of=2]  {};

    \path (0) edge              node [right]{Attack Component 1} (1)
              edge              node [left]{Attack Component 2} (2)
          (2) edge node {Goal} (8)
          (1) edge node {Goal} (5);

  \end{tikzpicture}
  }
  \caption{Attack Graph}
  \label{sfig:AG_OR_rad}
\end{subfigure}
\caption{OR Radical}
\label{fig:OR_rad}
\end{figure}

\begin{itemize}
\end{comment}

